BiSPARCs for Unsourced Random Access in Massive MIMO

This paper considers the massive MIMO unsourced random access problem in a quasi-static Rayleigh fading setting. The proposed coding scheme is based on a concatenation of a "conventional" channel code (such as, e.g., LDPC) serving as an outer code, and a sparse regression code (SPARC) serving as an inner code. The scheme combines channel estimation, single-user decoding, and successive interference cancellation in a novel way. The receiver performs joint channel estimation and SPARC decoding via an instance of a bilinear generalized approximate message passing (BiGAMP) based algorithm, which leverages the intrinsic bilinear structure that arises in the considered communication regime. The detection step is followed by a per-user soft-input-soft-output (SISO) decoding of the outer channel code in combination with a successive interference cancellation (SIC) step. We show via numerical simulation that the resulting scheme achieves stat-of-the-art performance in the massive connectivity setting, while attaining comparatively low implementation complexity.

==> sections/detection.tex <==
\section{Signal Detection}\label{sec:detection}
In this section, we develop message-passing based detector for the detection of the binary vectors $\mathbf{c}_k$. To this end we make use of the concepts of approximate message passing to derive tractable message updates and leverage the bilinear structure of the transmission model to facilitate user detection. We furthermore couple the detection algorithm with a \ac{SISO} decoder for the outer code in a \textit{turbo like} fashion and a successive interference cancellation step in which we substract successfully decoded codewords from the receive signal, thereby iteratively reducing the detection complexity. 

\subsection{Bilinear Formulation}
Consider the received signal $\mathbf{Y}$ defined in \eqref{eq:system_model}, the goal of the receiver is to detect the binary vectors $\hat{\mathrm{C}}=[\hat{\mathbf{c}}_{1},\ldots,\hat{\mathbf{c}}_{\Ka}]$ and subsequently decode the transmitted messages to output the message list $\hat{\mathcal{L}}:=\{\hat{W}_1,\ldots,\hat{W}_{\Ka}\}$. Given the concatenated coding scheme described in Section~\ref{sec:encoding}, in which an outer channel code is applied to $W_k$, the decoding step can highly benefit from a probabilistic estimation of $P_{\mathbf{c}_k\vert \mathbf{Y}}(\mathbf{s}_k\vert \mathbf{Y})\triangleq P_{W_k\vert \mathbf{Y}}(W_k\vert \mathbf{Y})$ since most high performance channel codes require soft inputs of the marginalized posterior estimates of code symbols. 

Given \eqref{eq:system_model}, the posterior distribution of the unknowns $\mathbf{C}$ and $\mathbf{H}$ given $\mathbf{Y}$ is given by
\begin{equation}
    P_{\mathbf{C},\mathbf{H}|\mathbf{Y}}(\mathbf{C},\mathbf{H}|\mathbf{Y})\propto P_{\mathbf{Y}|\mathbf{Z}}(\mathbf{Y}|\mathbf{Z})P_{\mathbf{C}}(\mathbf{C})P_{\mathbf{H}}(\mathbf{H}), \label{eq:posterior_system_model}
\end{equation}
with $\mathbf{Z}=\mathbf{A}\mathbf{C}\mathbf{H}^\mathrm{T}$. The posterior distribution in \eqref{eq:posterior_system_model} is composed of the likelihood distribution of the receive signal
\begin{equation}
    P_{\mathbf{Y}|\mathbf{Z}}(\mathbf{Y}|\mathbf{Z})= \prod\limits_{t=1}^T\prod\limits_{m=1}^M P_{y_{tm}\vert z_{tm}}(y_{tm}\vert z_{tm})
\end{equation}
where under the assumption of AWGN receive noise and independent antenna elements we have
\begin{equation}
    P_{y_{tm}\vert z_{tm}}(y_{tm}\vert z_{tm})=\mathcal{CN}( z_{mt}; y_{mt},\sigma^2).
\end{equation}
For Rayleigh block fading of coherence length $T$ and independent antenna elements, the prior distribution of the unknown channels $\mathbf{H}$ is given by
\begin{equation}
    P_{\mathbf{H}}(\mathbf{H})=\prod\limits_{k=1}^{\Ka}\prod\limits_{m=1}^M P_{h_{km}}(h_{km})
\end{equation}
with $(\forall k,m)\;P_{h_{km}}(h_{km})=\CN{h_{km}}{0}{1}$.
Given the section wise partitioned code structure of \ac{SPARC} encoding, the prior distribution of the SPARC encoded binary vectors is given by
\begin{equation}
    P_{\mathbf{C}}(\mathbf{C})=\prod\limits_{k=1}^{\Ka}\prod\limits_{l=1}^{L} P_{\mathbf{c}_k^{(l)}}(\mathbf{c}_k^{(l)})
\end{equation}
where with the definition from \eqref{eq:sparc_coder} we have
\begin{equation}
    P_{\mathbf{c}_k^{(l)}}(\mathbf{c}_k^{(l)})=\frac{1}{Q}\sum\limits_{n=1}^{Q}\delta(c_{nk}^{(l)}-1)\prod\limits_{j\neq n} \delta(c_{jk}^{(l)}).\label{eq:subvector_pmf}
\end{equation}
Given the prior distributions, the quantity of interest is the marginal posterior distribution of the binary entries 
\begin{equation}
    P_{c_{nk}|\mathbf{Y}}(c_{nk}^{(l)}|\mathbf{Y})    \propto\sum_{\mathbf{C}/c_{nk}^{(l)}}\int_{d\mathbf{H}}P_{\mathbf{Y}|\mathbf{Z}}(\mathbf{Y}|\mathbf{Z})P_{\mathbf{C}}(\mathbf{C})P_{\mathbf{H}}(\mathbf{H})\label{eq:marginal_posterior}
\end{equation}
where $\mathbf{C}/c_{nk}^{(l)}$ denotes the matrix $\mathbf{C}$ with omitted element $\mathbf{c}_{nk}^{(l)}$. The marginalized posterior probability of the binary vector elements can be translated to the posterior distribution of code symbols as  
\begin{equation}
    P_{c_{nk}|\mathbf{Y}}(c_{nk}^{(l)}=1|\mathbf{Y})\triangleq P_{W_k^{(l)}|\mathbf{Y}}(W_k^{(l)}=n|\mathbf{Y})    
\end{equation}
which we passed in a subsequent iteration step as symbol priors to a soft-input-soft-output (SISO) decoder of the outer channel code.

\subsection{Factor Graph Representation}
The marginalization of the posterior distribution as stated in \eqref{eq:marginal_posterior} is computationally intractable and can generally only be solved approximately with deterministic algorithms using algorithms based on loopy belief propagation (LBP) \cite{bishop1} (also known as message passing). LBP exploits the factorizable structure of the posterior distribution \eqref{eq:posterior_system_model} to reduce the complexity of computing the marginals. To derive the message passing messages for a given distribution, it is convenient to represent the factorized distribution as so-called factor graphs. In factor graphs, the factorized distributions are represented by factor nodes, which we represent by filled squares, that are connected with their associated arguments or also variable nodes, which we represent by empty circles. The connections are represented by lines.

The bilinear and affine relation between the random variables $\mathbf{Z}$, $\mathbf{C}$ and $\mathbf{H}$, however greatly diminish the factorizability of \eqref{eq:posterior_system_model} and thus makes the computation of the messages involving these factor nodes intractable. To circumvent this problem we will resort to a variant of the LBP algorithm known as approximate message passing algorithms \cite{parker_bilinear_2014, Donoho, Rangan11,rangan17}, which reduce the computational complexity of LBP by approximating the messages using central limit theorem (CLT) arguments and first-order approximations. To derive the messages we split the factor graph corresponding to \eqref{eq:posterior_system_model} into two separate factor graphs. The first factor graph depicted in Fig.~\ref{fig:weak_factor_graph} contains all the nodes connected by weak edges, for which we derive approximate message updates. The second factor graph depicted in Fig.~\ref{fig:strong_factor_graph} contains all the strong edges for which we derive exact message updates. We connect both factor graphs in an iterative turbo-like fashion, where we first iterate over the weak edges until convergence and pass the computed likelihoods to the strong edges for the sparsity update. 

\begin{figure}[hbt!]
    \centering
    \input{tikz/factorgraph.tex}
    \caption{Factor graph with weak edges.}
	\label{fig:weak_factor_graph}
\end{figure}

\subsubsection{Message updates for the weak edges}
The message passing algorithm on the factor graph in Fig.~\ref{fig:weak_factor_graph} is described as following. Denote by $\Delta^i_{a\rightarrow b}(\cdot)$ the message from node $a$ to $b$ in iteration $i$, and by $\Delta^i_c(\cdot)$ the marginal posterior computed at variable node $c$ in iteration $i$. Applying the sum-product rules, we obtain the following messages and marginal posteriors
For variable nodes $\{w_{nm}\}$:
\begin{equation}
\M{z_{tm}}{f_{nm}^w}{i}{w_{nm}}\propto \int\limits_{w_{lm}\neq w_{nm}} f^z_{tm} \prod_{l\neq n}\M{f_{lm}}{z_{tm}}{i}{w_{lm}}\label{eq:first_message}
\end{equation}
\begin{equation}
\M{f_{nm}^w}{z_{tm}}{i+1}{w_{nm}} \propto f^w_{nm}(i)\prod_{l\neq t}\M{z_{lm}}{f_{nm}^w}{i}{w_{nm}}\label{eq:first_update}
\end{equation}
For variable nodes $\{h_{km}\}$:
\begin{equation} 
    \M{f_{nm}^w}{h_{km}}{i}{h_{km}} \propto \int\limits_{\substack{c_{nk} \\ h_{lm}\neq h_{km}}} \prod_{k=1}^{\Ka}\M{c_{nk}}{f_{nm}^w}{i}{s_{nk}}\times\prod_{l\neq k}\M{h_{lm}}{f_{nm}^w}{i}{h_{lm}}\prod_{t=1}^T\M{z_{tm}}{f_{nm}^w}{i}{w_{nm}}\label{eq:second_message}
\end{equation}
\begin{equation}
    \M{h_{km}}{f_{nm}^w}{i+1}{h_{km}} \propto  f^h_{km}(i)\prod_{l\neq n}\M{f_{lk}^h}{h_{km}}{i}{h_{km}}\label{eq:second_update}
\end{equation}
For variable nodes $\{c_{nk}\}$:
\begin{equation}
        \M{f_{nm}^w}{c_{nk}}{i}{c_{nk}}\propto\int\limits_{\substack{h_{lm} \\ c_{nl}\neq c_{nk}}} \prod_{k=1}^{\Ka}\M{h_{km}}{f_{nm}^w}{i}{h_{km}}\times\prod_{l\neq k}\M{c_{nl}}{f_{nm}^w}{i}{c_{nl}}\prod_{t=1}^T\M{z_{tm}}{f_{nm}^w}{i}{w_{nm}}
    \label{eq:third_message}
\end{equation}
\begin{equation}
    \M{c_{nk}}{f_{nm}^w}{i+1}{c_{nk}}\propto f^c_{nk}(i)\prod_{l\neq n}\M{f_{lk}}{c_{nk}}{i}{c_{nk}}\label{eq:third_update}
\end{equation}
Message computations require high-dimensional integration and normalization. To yield tractable messages, we resort to approximately calculate these messages by leveraging the general idea of the AMP framework \cite{parker_bilinear_2014,Donoho,Rangan11}. The details of the messages are presented in Appendix~\ref{sec:message-derivation}. To facilitate derivation of the approximations, we introduce auxiliary random variables which are characterized by their mean and variance quantities which we summarize in Table~\ref{tbl:updates}. Following the AMP principle, we derive the messages in the large-system limit, i.e, $N,K,M,T\rightarrow \infty$ with fixed ratios for $M/N$, $K/N$ and $T/N$. Without loss of generality, we assume that $h_{km}$ scales as $O(1/\sqrt{M})$ and $C_{tn}$ scales as $O(1/\sqrt{T})$, other quantities scale as $O(1)$.
\input{tables/message_approximations.tex}
\begin{subequations}
    \label{eq:auxiliary}
    \begin{align}
        \hat{h}_{km}(i+1)&=\int_{h_{km}}h_{km}\Delta_{h_{km}}^i(h_{km})\label{eq:channel1},\\
        v_{km}^{h}(i+1)&=\int_{h_{km}}h_{km}^2\Delta_{h_{km}}^i(h_{km})-\vert\hat{h}_{km}(i+1)\vert^2\label{eq:channel2},\\
        \hat{c}_{nk}(i+1)&=\int_{c_{nk}}c_{nk}\Delta_{c_{nk}}^i(c_{nk})\label{eq:bcode1},\\
        v_{nk}^{c}(i+1)&=\int_{c_{nk}}c_{nk}^2\Delta_{c_{nk}}^i(c_{nk})-\vert\hat{c}_{nk}(i+1)\vert^2\label{eq:bcode2}
    \end{align}
\end{subequations}
Given the Rayleigh fading assumption, \eqref{eq:channel1} and \eqref{eq:channel2} are be readily given by
\begin{subequations}
    \begin{align}
        \hat{h}_{km}(i+1)&=\frac{\hat{r}_{km}(i)}{1+v_{km}^r(i)}\label{eq:channel_update},\\
        v_{km}^{h}(i+1)&=\frac{v^r_{km}(i)}{1+v_{km}^r(i)}\label{eq:channel_var_update},
    \end{align}
\end{subequations}
and for the binary codewords in \eqref{eq:bcode1} and \eqref{eq:bcode2}, we get
\begin{subequations}
    \begin{align}
         \hat{c}_{nk}(i+1)&=\frac{1}{1+\frac{(1-\epsilon_{nk})}{\epsilon_{nk}}\exp(\frac{1-2\mathrm{Re}\{\hat{q}_{nk}(i)\}}{v^{q}_{nk}(i)})}\label{eq:code_update},\\
        v_{nk}^{c}(i+1)&=\frac{\frac{(1-\epsilon_{nk})}{\epsilon_{nk}}\exp(\frac{1-2\mathrm{Re}\{\hat{q}_{nk}(i)\}}{v^{q}_{nk}(i)})}{(1+\frac{(1-\epsilon_{nk})}{\epsilon_{nk}}\exp(\frac{1-2\mathrm{Re}\{\hat{q}_{nk}(i)\}}{v^{q}_{nk}(i)}))^2}\label{eq:code_var_update}
    \end{align}
\end{subequations}

%\begin{table}[hbt!]
%\caption{Factor graph with strong edges.\label{tbl:strong_factor_graph_table}}
%\centering
%\begin{tabular}{l | l | l } 
    %\hline
    %Factor & Distribution & Exact Form\\ 
    %\hline
    %$d_{nk}^{s,(l)}$ &  $ P_{\mathbf{s}_k^{(l)}\vert \lambda_k}(\mathbf{s}_k^{(l)}\vert\lambda_k)$& defined in \eqref{eq:subvector_pmf}\\
%    $d_{k}^{\lambda}$ & $P_{\lambda_k}(\lambda_k)$ & defined in \eqref{eq:ua_pmf}\\
%    $d_{km}^{h}$ & $\Delta_{h_{km}}^i(h_{km})$&defined in \eqref{eq:second_update}\\
%    \hline
%\end{tabular}
%\end{table}

\subsubsection{Message Updates of Strong Edges}

After iterating through the weak edges, we pass along the strong edges to the binary codeword variables by passing the messages
\begin{equation}
    \Delta_{c_{nk}\rightarrow f_{nk}^c}^i(c_{nk})\triangleq d^c_{nk}(c_{nk})=\mathcal{CN}(c_{nk};\hat{q}_{nk}(i),v^q_{nk}(i))
\end{equation}
Given \eqref{eq:subvector_pmf} we have $d^c_{lk}\triangleq P_{\mathbf{c}_k^{(l)}}(\mathbf{c}_k^{(l)})$ which we marginalize with respect to $c_{nk}^{(l)}$, i.e.,
%$\mathbf{c}_k^{(l)}$ to get the subsequent messages to the activity variable $\lambda_k$
\begin{equation}
    \Delta_{d^c_{kl}\rightarrow c_{nk}^{(l)}}^i(c_{nk}^{(l)})=\begin{cases}
        \Delta_{c_{nk}^{(l)}\rightarrow d_{lk}^c}^i(1)\prod\limits_{j\neq n} \Delta_{c_{jk}^{(l)}\rightarrow d_{lk}^c}^i(0)&c_{nk}^{(l)}=1\\
        \frac{1}{Q}\sum\limits_{j\neq n}\Delta_{c_{jk}^{(l)}\rightarrow d_{lk}^c}^i(1) \prod\limits_{v\neq j} \Delta_{c_{uk}\rightarrow d_{lk}^c}^i(0)&c_{nk}^{(l)}=0
    \end{cases}
\end{equation}
%\begin{equation}
 %   \Delta_{d^c_{kl}\rightarrow \lambda_k}^i(\lambda_k)=\begin{cases}
  %      \frac{1}{M}\sum\limits_n \Delta_{c_{nk}^{(l)}\rightarrow d_{lk}^c}^i(1)\prod\limits_{j\neq n} \Delta_{c_{jk}^{(l)}\rightarrow d_{lk}^c}^i(0)&\lambda_k=1\\
   %     \prod\limits_n \Delta_{c_{nk}\rightarrow d_{lk}^c}^i(0)&\lambda_k=0
%    \end{cases}
%\end{equation}
%which we represent in log-likelihood ratio form as
%\begin{equation}
    %\mathrm{LLR}_{d^c_{lk}\rightarrow c_{nk}^{(l)}}^i=\log \sum_n %\exp(\frac{2\hat{q}_{nk}^{(l)}(i)-1}{v^{q,(l)}_{nk}(i)}) -\log M.
%\end{equation}

%For the message from the channel side we have
%\begin{equation}
%\Delta_{d^h_{km}\rightarrow \lambda_k}^i(\lambda_k)=\lambda_k\mathcal{CN}(0;\hat{r}_{km}(i),v^k_{km}(i)+1)+(1-\lambda_k)\mathcal{CN}(0;\hat{r}_{km}(i),v^k_{km}(i))
%\end{equation}
%conveniently written as log-likelihood ratios
%\begin{equation}
 %   \mathrm{LLR}_{d^h_{km}\rightarrow \lambda_k}^i=\log\frac{v^k_{km}(i)}{v^k_{km}(i)+1}+\frac{\vert \%hat{r}_{km}(i)\vert^2}{v^k_{km}(i)(v^k_{km}(i)+1)}
%\end{equation}
%The user activity belief update for the next iteration can now be given by
%\begin{equation}
%\mathrm{LLR}_{\lambda_k}^{i+1}=\log \rho_k/(1-\rho_k)+\sum_l \mathrm{LLR}_{h^c_{kl}\rightarrow \lambda_k}^i + \sum_m \mathrm{LLR}_{d^h_{km}\rightarrow \lambda_k}^i
%\end{equation}
%from which the probability of activation can be derived as
%\begin{equation}
 %   \hat{\rho}_k^{i+1}\triangleq (1+\exp -\mathrm{LLR}_{\lambda_k}^{i+1})^{-1}
%\end{equation}
%After passing the belief updates for the user activity $\hat{\rho}_k^{i+1}$ 
from which we compute the belief updates for the binary vector elements by marginalizing over $d_{lk}^c$ which results in following messages
\begin{equation}
     \Delta_{d^c_{lk}\rightarrow c_{nk}^{(l)}}^{i+1}(c_{nk}^{(l)}=1)\triangleq \hat{\epsilon}_{nk}^{(l)}(i+1)\triangleq \hat{\epsilon}_{nk}^{i+1}=    \left(1+Q\sum_n \exp(\frac{1-2\mathrm{Re}\{\hat{q}^{(l)}_{nk}(i)\}}{v^{q,(l)}_{nk}(i)})\right)^{-1}.
\end{equation}
The beliefs $\hat{\epsilon}_{nk}^{i+1}$ are passed as extrinsic information to the outer \ac{SISO} channel for single user decoding.

\subsection{The Overall Algorithm}

\begin{figure}[hbt!]
\centering
\input{tikz/detection.tex}
\caption{Turbo-like iteration between modules.\label{fig:scheme}}
\end{figure}

In Algorithm~\ref{alg:bigamp} we summarize the detection algorithm.
\input{sections/algorithm.tex}


%\begin{table}[h]
 %   \caption{Notation of the Factor nodes connected with weak edges.}
 %  \label{fig:weak_factor_graph_table}
 %   \centering
 %   \begin{tabular}{l | l | l } 
 %   \hline
 %   Factor & Distribution & Exact Form\\ 
 %   \hline
 %   $f_{nm}^w$ & $P(w_{tm}\vert s_{nk},h_{km})$ & $\delta(w_{tm}-\sum_ks_{nk}h_{km})$\\
 %   $f_{tm}^z$ & $P_{y_{tm}\vert z_{tm}}(y_{tm}\vert z_{tm})$ & $\mathcal{CN}(z_{tm};y_{tm},\sigma^2)$\\
 %   $f_{nk}^c$ & $P_{c_{nk}}(c_{nk})$&$\epsilon_{nk}\delta(c_{nk}-1)+(1-\epsilon_{nk})\delta(c_{nk})$\\
 %   $f_{km}^h$ & $P_{h_{km}}(h_{km})$&$\rho_k \mathcal{CN}(h_{km};0,1)+(1-\rho_k)\delta(h_{km})$\\
 %   \hline
 %   \end{tabular}
%\end{table}

%\subsection{Notes on User Activity Estimation}
%Our formulation 

==> sections/detection_scheme.tex <==
\begin{algorithm}[h]
\caption{BiGAMP for Detection. }\label{alg:bigamp}
\allowdisplaybreaks
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\STATE \textbf{Input}: $\mathbf{Y}$, $\mathbf{A}$, $t_{\mathrm{Max}}$
\STATE \textbf{Initialize:}\\
$\forall (n,k):\epsilon_{nk}=\frac{1}{Q},\;\forall(n,k):\hat{c}_{nk}\sim\mathrm{Bernoulli}(\frac{1}{Q})$\\
$\forall (k,m):\hat{h}_{nk}(0)=0,\;\forall (k,m):\hat{v}_{nk}^h(0)=0$\\
\FOR {$i=1$ to $t_{\mathrm{Max}}$} 
\STATE $\theta_{nm}^{(i)}=\sum_{t=1}^T a_{tn}^*\mu_{tm}^{z,(i)}+\mu_{nm}^{x,(i)}$\\
\STATE $\mu_{nm}^{x,(i)}=\frac{\theta_{nm}^{(i)}\nu_{nm}^{x,(i)}+\mu_{nm}^{x,(i)}\nu_{nm}^{z,(i)}}{\nu_{nm}^{x,(i)}+\nu_{nm}^{z,(i)}}$\\
\STATE $\nu_{nm}^{x,(i)}=\frac{\nu_{nm}^{z,(i)}\nu_{nm}^{x,(i)}}{\nu_{nm}^{z,(i)}+\nu_{nm}^{x,(i)}}$\\
\STATE $\nu_{nm}^{z,(i)}=\sigma^2+\frac{1}{T}\sum_{n=1}^N\nu_{nm}^{x,(i+1)}$\\
\STATE $\mu_{tm}^{z,(i)}=y_{tm}-\sum_{n}a_{tn}\mu_{nm}^{x,(i)}$\\
\STATE $\mu_{tm}^{z,(i)}=\mu_{tm}^{z,(i)}+\frac{\mu_{tm}^{z,(i)}}{T}\sum_{n=1}^NF(\theta_{nm}^{(i)},\nu_{nm}^{z,(i)})$\\
\STATE $\nu^{p,(i)}_{nm}=\sum_k\vert\mu^{c,(i)}_{nk}\vert^2\nu^{h,(i)}_{km}+\nu^{c,(i)}_{nk}\vert \mu^{h,(i)}_{km}\vert^2\nonumber+\nu^{c,(i)}_{nk}\nu^{h,(i)}_{km}$\\
\STATE $\mu^{p,(i)}_{nm}=\sum_k \mu^{c,(i)}_{nk}\mu^{h,(i)}_{km}-\mu^{\alpha,(i)}_{nk}\vert\mu^{c,(i)}_{nk}\vert^2 \nu^{h,(i)}_{km}$\\
\STATE $\nu_{nm}^{\alpha,(i)}=(\nu^{p,(i)}_{nm}+\nu_{nm}^{x,(i)})^{-1}$\\
\STATE $\mu^{\alpha,(i)}_{nm}=\frac{\mu_{nm}^{x,(i)}-\mu^{p,(i)}_{nm}(i)}{\nu^{p,(i)}_{nm}+\nu^{x,(i)}_{nm}}$\\
\STATE $\nu_{km}^{r,(i)}=(\sum_n \vert\mu^{c,(i)}_{nk}\vert^2\nu_{nm}^{\alpha,(i)})^{-1}$\\
\STATE $\mu^{r,(i)}_{km}=\mu^{h,(i)}_{km}(1-\nu^{r,(i)}_{km}\sum_n \nu^{c,(i)}_{nk}\nu_{nm}^{\alpha,(i)})$\\
\STATE $\mu^{r,(i)}_{km}=\mu^{r,(i)}_{km}+\nu^{r,(i)}_{km}\sum_n\mu^{c,(i),*}_{nk}\mu^{\alpha,(i)}_{nm}$\\
\STATE $\nu^{q,(i)}_{nk}=(\sum_m\vert\mu^{h,(i)}_{km}\vert^2\nu_{nm}^{x,(i)})^{-1}$\\
\STATE $\mu^{q,(i)}_{nk}=\mu^{c,(i)}_{nk}(1-\nu_{nk}^{q,(i)}\sum_m \nu^{h,(i)}_{km}\nu_{nm}^{x,(i)})$\\
\STATE $\mu^{q,(i)}_{nk}=\mu^{q,(i)}_{nk}+\nu_{nk}^{q,(i)}\sum_m\mu^{h,(i),*}_{km}\mu^{x,(i)}_{nm}$
\STATE $\mu^{h,(i+1)}_{km}=\frac{\mu^{r,(i)}_{km}}{\nu_{km}^{r,(i)}+1}$\\
\STATE $\nu_{km}^{h,(i+1)}=\frac{\nu_{km}^{r,(i)}}{\nu_{km}^{r,(i)}+1}$\\
\STATE $\mu^{c,(i+1)}_{nk}=$\\
\STATE $\nu_{nk}^{c,(i+1)}=$
\ENDFOR
\end{algorithmic}  
\end{algorithm}

==> tables/message_approximations.tex <==
\begin{table*}[hbt!]
    \centering
    \caption{Message approximation. \label{tbl:updates}}
    \begin{tabular}{l | l | l | l} 
    \hline
    Message/Posterior & Mean & Variance & PDF \\ 
    \hline
    $\M{f_{nm}^w}{z_{tm}}{i}{w_{nm}}$ & $\hat{w}_{nm}(i)$   & $v^w_{nm}(i)$   & $\mathcal{CN}(w_{nm};\hat{w}_{nm}(i),v^w_{nm}(i))$\\
    $\M{h_{km}}{f_{nm}^w}{i}{h_{km}}$ & $\hat{h}_{km,n}(i)$ & $v^h_{km,n}(i)$ & $\mathcal{CN}(h_{km};\hat{r}_{km,n}(i),v^r_{km,n}(i))f^h_{km}(i)$\\
    $\M{c_{nk}}{f_{nm}^w}{i}{c_{nk}}$ & $\hat{c}_{nk,n}(i)$ & $v^c_{nk,n}(i)$ & $\mathcal{CN}(c_{nk};\hat{q}_{nk,n}(i),v^q_{nk,n}(i))f^c_{nk}(i)$\\
    $\Delta_{h_{km}}^i(h_{km})$     & $\hat{h}_{km}(i)$   & $v^h_{km}(i)$   & $\mathcal{CN}(h_{km};\hat{r}_{km}(i),v^r_{km}(i))f^h_{km}(i)$\\
    $\Delta_{c_{nk}}^i(c_{nk})$     & $\hat{c}_{nk}(i)$   & $v^c_{nk}(i)$   & $\mathcal{CN}(c_{nk};\hat{q}_{nk}(i),v^q_{nk}(i))f^c_{nk}(i)$\\
    \hline
    \end{tabular}
\end{table*}

==> tikz/first.tex <==
\draw[fill=white, fill opacity=1] rectangle (\WIDTH,\HEIGHT);
\def\C{{\WIDTH/2-1.25,\HEIGHT/2},{\WIDTH/2-1.25,\HEIGHT*.75}, {\WIDTH/2-1.25,\HEIGHT*.25}}
\def\W{{\WIDTH/2,\HEIGHT*.15}, {\WIDTH/2,\HEIGHT/2}, {\WIDTH/2,\HEIGHT*.85}}
\def\Z{{\WIDTH/2+1,\HEIGHT*.25}, {\WIDTH/2+1,\HEIGHT*.5}, {\WIDTH/2+1,\HEIGHT*.75}}

\readarray\CLABELS\CLABELSA[1,3]
\readarray\CLABELSF\CLABELSFA[1,3]

\readarray\ZLABELS\ZLABELSA[1,3]
\readarray\ZLABELSF\ZLABELSFA[1,3]
\readarray\WLABELSF\WLABELSFA[1,3]

\drawFullyConnection{\W}{\C}

\draw[black,thin] (\WIDTH/2+1,\HEIGHT*.25) -- (\WIDTH/2,\HEIGHT*.15);
\draw[black,thin] (\WIDTH/2+1,\HEIGHT*.5)  -- (\WIDTH/2,\HEIGHT/2);
\draw[black,thin] (\WIDTH/2+1,\HEIGHT*.75) -- (\WIDTH/2,\HEIGHT*.85);

\foreach \i [count=\xi] in \W {
    \drawFactor{\i}{\WLABELSFA[1,\xi]};
}

\foreach \i [count=\xi] in \C {
    \drawVariableFactor{\i}{-\FVDIST}{0}{\CLABELSA[1,\xi]}{\CLABELSFA[1,\xi]};
}

\foreach \i [count=\xi] in \Z {
    \drawVariableFactor{\i}{\FVDIST}{0}{\ZLABELSA[1,\xi]}{\ZLABELSFA[1,\xi]};
}
    
